Arrow Matrix Decomposition: A Novel Approach for Communication-Efficient Sparse Matrix Multiplication

We propose a novel approach to iterated sparse matrix dense matrix multiplication, a fundamental computational kernel in scientific computing and graph neural network training. In cases where matrix sizes exceed the memory of a single compute node, data transfer becomes a bottleneck. An approach based on dense matrix multiplication algorithms leads to suboptimal scalability and fails to exploit the sparsity in the problem. To address these challenges, we propose decomposing the sparse matrix into a small number of highly structured matrices called arrow matrices, which are connected by permutations. Our approach enables communication-avoiding multiplications, achieving a polynomial reduction in communication volume per iteration for matrices corresponding to planar graphs and other minor-excluded families of graphs. Our evaluation demonstrates that our approach outperforms a state-of-the-art method for sparse matrix multiplication on matrices with hundreds of millions of rows, offering near-linear strong and weak scaling.

==> artifacts.tex <==
\section{Artifact Description}

% NOTE: This text will be inserted into the ad/ae form and is here just for reference.
% The AD/AE appendix will be generated from the responses to the form

\subsection{Artifact Identification}

%START_LATEX

We propose a novel approach for iterated sparse matrix dense matrix multiplication, a key computation in scientific computing and graph neural network training. Our approach addresses the challenge of data movement in scenarios where matrices are too large to fit into a single compute node's memory. We decompose the sparse matrix into a small number of structured matrices called "arrow" matrices, connected by permutations, enabling communication-avoiding multiplications. Our evaluation demonstrates good strong and weak scaling, outperforming 1.5D decomposition, a state-of-the-art method for sparse matrix multiplication on a set of matrices from the SuiteSparse matrix collection with tens to hundreds of millions of rows.

Our computational artifacts include (A) our codes and (B) datasets. These artifacts enable the reproducibility of our experiments by providing all code and data necessary to run our experiments and produce the figures and tables from our evaluation.

\paragraph{A. Codes}

Our code artifacts come from five categories:

\begin{description}
    \item[A0] Arrow Matrix Decomposition Code, which performs the decomposition into arrow matrices.
    \item[A1] MPI SpMM Implementation using the Arrow Matrix Decomposition.
    \item[A2] MPI SpMM Implementation of the 1.5D Baseline.
    \item[A3] Bandwidth of RCM-permuted matrices. Using the scipy.sparse implementation of the reverse Cuthill-McKee algorithm, this code computes the RCM permutations of the datasets. Then it computes their bandwidth and visualizes the sparsity structure.
    \item[A4] Dataset Analysis code. This code computes graph statistics for each dataset, such as the number of nodes and edges and the minimum, maximum, and average degree. 
\end{description}

The source code can be found at the following link: \\ \url{https://zenodo.org/badge/latestdoi/630814722}.

\paragraph{B. Datasets}

We provide the input datasets in two formats: (\textbf{B1}) compressed sparse row (numpy .npz) and (\textbf{B2}) a graph format (igraph pickled).
Moreover, we provide the decomposed matrices in numpy .npz/.npy format (\textbf{B3}). For all dataset formats, we provide data loader functions that are integrated with our experimental workflow.

All these preprocessed datasets can be found under the following link: \url{https://doi.org/10.5281/zenodo.7850816}.
%
The raw data can be downloaded from the following links:

\noindent
\url{https://suitesparse-collection-website.herokuapp.com/MAWI}

\noindent
\url{https://suitesparse-collection-website.herokuapp.com/GenBank}

\noindent
\url{https://suitesparse-collection-website.herokuapp.com/LAW/} \\

All datasets are available under a CC v 4.0 license \footnote{Timothy A. Davis and Yifan Hu. 2011. The University of Florida Sparse Matrix Collection. ACM Transactions on Mathematical Software 38, 1, Article 1 (December 2011), 25 pages. DOI: \url{https://doi.org/10.1145/2049662.2049663}} \footnote{\url{https://creativecommons.org/licenses/by/4.0/}}

%STOP_LATEX


%START_LATEX
We begin by describing the overall workflows and how their results relate to the submission. Then, we proceed by describing how to run the individual code artifacts \textbf{A0}-\textbf{A4}.

\section{Experimental Workflow}
The experiments can be divided into two workflows, which can be reproduced independently:

\begin{description}
    \item[E1] Evaluation of the arrow matrix decomposition.
    \item[E2] Evaluation of the SpMM performance.
\end{description}

\subsection{Evaluation of Arrow Matrix Decomposition}

This workflow requires artifacts \textbf{A0}, \textbf{A3}, \textbf{A4}, \textbf{B1}, and \textbf{B2}.
\begin{enumerate}
    \item Download the source code.
    \item Download the datasets, \emph{make a copy}, and place them under 'datasets' in the root directory of the code. This workflow modifies the datasets, so if you want to use the original datasets you need to make a copy of the datasets or download them again before running \textbf{E2}.
    \item Run \textbf{A0}
    \item Run \textbf{A3}
    \item Run \textbf{A4}
\end{enumerate}
It takes approximately 8-12 hours to run this workflow.

%
The expected outcome of running \textbf{A0} is the matrices and permutations necessary for creating Figure 1 and part of the data for Figure 4 and Table 3. 
To generate Figure 1, use the script in
\begin{verbatim}
    src/evaluation/block_analysis_main.py
\end{verbatim}
and to generate the data for Figure 4, use the script in 
\begin{verbatim}
    src/evaluation/graph_stats.py
\end{verbatim}

Running \textbf{A3} provides the rest of the data for Table 3.

Running \textbf{A4} provides the data for Table 2.

\subsection{Evaluation of SpMM performance}

This workflow requires artifacts \textbf{A1}, \textbf{A2}, \textbf{B1} and \textbf{B3}. It takes approximately 2000 compute node hours to run the experiment workflow. If all experiments were run concurrently, they would take less than half an hour to execute on comparable hardware.

\begin{enumerate}
    \item Download the source code, if you have not done so already.
    \item Create a \url{http://wandb.ai} account and note your API key.
    \item Download the datasets and place them under 'datasets' in the root direcrory of the code. 
    \item Run \textbf{A1} passing your wandb API key
    \item Run \textbf{A2} passing your wandb API key
\end{enumerate}
All experiments data is logged to wandb.ai\footnote{Experiment Tracking with Weights and Biases, 2020, \url{https://www.wandb.com/}, Lukas Bielewald}. The metric reported in the experiments, the time it takes to perform an SpMM iteration, is spmm\_time. This number is logged to the standard output as well, for each rank and iteration. Note that the logging to wandb.ai occurs after all processes have finished, while the logging to standard output occurs during the execution of the program.

Running the artifacts generates the data necessary to generate Figures 5, Figures 6, and the data for Table 4. After running the SpMM benchmarks \textbf{A1} and \textbf{A2}, run the script in 
\begin{verbatim}
    evaluation/strong_scaling_fig5_wandb.py
\end{verbatim}
to generate Figure 5 and the script in 
\begin{verbatim}
    evaluation/weak_scaling_fig6_wandb.py
\end{verbatim}
to generate Figure 6, and the script in 
\begin{verbatim}
    evaluation/eval_tab6_wandb.py
\end{verbatim}
to generate the results for Table 4. To run the scripts, set the API\_KEY global variable.

\section{Running the Code Artifacts}

Next, we provide further instructions on how to run our code.

\paragraph{A0. Decomposition Code}

%The decomposition code is implemented in src/preprocessing/arrowdecomposition.py. 
The preprocessing of datasets is done using the
\begin{verbatim}
    src/preprocessing/decomposition_main.py
\end{verbatim}
python script. The script has two optional arguments:
\begin{itemize}
    \item -f <path/to/directory> the dataset folder containing all the downloaded datasets in its subdirectories. By default, the directory is '/datasets/'
    \item -n <dataset1 dataset2> a list of dataset names to preprocess. By default, this is a list of all datasets we used.
\end{itemize}
For each dataset, the script will save all corresponding files into the subdirectories, which could be used for running the SpMM algorithm (\textbf{A1}) later.

The estimated runtime is between $10$ minutes and $60$ minutes per dataset.


\paragraph{A1. SpMM using Arrow Matrix Decomposition}

The implementation of our SpMM algorithm can be found in src/arrow\_main\_mpi.py, src/arrow\_mpi.py, and src/arrow\_dec\_mpi.py. The entry point is the src/arrow\_main\_mpi.py script and it can be executed as follows:
\begin{verbatim}
    mpirun -n <N> python ./src/arrow_main_mpi.py <args>
\end{verbatim}
where \textit{<N>} is the number of MPI processes and \textit{<args>} are arguments that customize the script's execution. To replicate the experiments, the following arguments are relevant:

\begin{itemize}
    \item -f <path/to/file>: The absolute or relative path to the file containing the sparse matrix A. This name excludes any suffixes that are appended to the dataset name.  The name of the dataset is the one that matches its name in the SuiteSparse matrix collection. For example, to run on the webbase dataset, pass './datasets/webbase-2001/webbase-2001'
    \item -c <number-of-X-columns>: The number of columns in matrices \mat{X} and \mat{Y}. The default value is \textit{128}.
    \item -w <width>: The arrow width of the decomposition.
    \item -z <number-of-iterations>: How many times to execute the SpMM operation. The default value is \textit{10}.
    \item -i [cpu|gpu]”: Whether to execute the code on the CPU or GPU. The default is cpu.
    %\item -s <seed>: The seed for the pseudo-random number generated used to initialize data. The default value is \textit{42}.
    \item -k <wandb-key>: The API key for your wandb.ai profile. %If you do not have a wandb.ai account, pass None to log the data in anonymous mode.
    %\item 
\end{itemize}
Running the algorithm takes between $10$ and $20$ minutes, depending on the number of processes, columns, iterations, and the input graph.

For convenience, we provide two scripts that runs all the configurations required for replicating the experiments. They are located in /src/bash/arrow/run.sh and /src/bash/arrow/run.sh and assume that your system uses the SLURM batch manager. The script takes a single argument, your wanb.ai API key. Running this script will use the preprocessed data from artifact \textbf{B3} in /datasets. If your data is in another directory, you might need to adapt those paths.

If you wish to use a different set of decompositions (constructed directly using \textbf{A0}), use the /bash/arrow\_mpi\_run\_custom.sh script. It takes an additional argument, the directory containing the decomposed matrices. Within this directory, the decomposed matrices for each dataset must reside within a directory that matches the name of the dataset. You can run a subset of the experiments by copying individual lines from this bash script.

If you are using a different system, you will need to adjust the batching scripts accordingly.

%If you wish to make a local test run of the algorithm on synthetic data, you can run the src/test\_arrrowmpi.py unit test. 

\paragraph{A2. SpMM 1.5D Baseline}

The baseline implementation can be found in src/spmm2d\_distr.py and can be executed similarly as our other SpMM code using:
\begin{verbatim}
    mpirun -n <N> python ./src/spmm2d_distr.py <args>
\end{verbatim}
The program takes the same arguments as our other SpMM code A1 except it does not need a width argument. In contrast to A1, the filename should be the .npz file that contains the A matrix. For example, to run on webbase, pass './datasets/webbase-2001/webbase-2001\_A.npz'.

Running the algorithm takes between $10$ and $20$ minutes, depending on the number of processes, columns, iterations, and the input graph.

\iffalse
\textit{args} are optional arguments that customize the script's execution:
\begin{itemize}
    \item -d [random|file]: Switches between generating a random sparse matrix A and one read from a file. The default value is \textit{file}.
    \item -f <path/to/file>: The absolute or relative path to the file containing the sparse matrix A. This parameter is used only when the script is called using \textit{-d file}. The default value is \textit{None}.
    \item -v <number-of-vertices>: Changes the number of vertices (rows or columns) of the random sparse matrix \mat{A}. The default value is \textit{100000}.
    \item -e <number-of-edges>: Changes the number of edges (number of non-zero values) of the random sparse matrix \mat{A}. The default value is \textit{1000000}.
    \item -t [float32|float64]: The datatype used for matrices \mat{A}, \mat{X}, and \mat{Y}. Even if the sparse matrix is read from a file, if this argument is set, it will override the datatype found in the file. The default value is \textit{float32}.
    \item -c <number-of-X-columns>: The number of columns in matrices \mat{X} and \mat{Y}. The default value is \textit{128}.
    \item -z <number-of-iterations>: How many times to execute the SpMM operation. The default value is \textit{10}.
    \item -i [cpu|gpu]”: Whether to execute the baseline on the CPU or GPU.
    \item -s <seed>: The seed for the pseudo-random number generated used to initialize data. The default value is \textit{42}.
\end{itemize}
\fi

The script takes a single argument, your wandb.ai API key. Running this script will use the data from artifact \textbf{B1} assuming it has been placed in the /datasets directory. If your data is in another directory, you might need to adapt those paths.

\paragraph{A3. Bandwidth of RCM-permuted matrices} 

The code to compute RCM permutations and analyze the resulting bandwidths (\textbf{A3}) can be found in 

\verb|./src/graphprocessing/rcm.py|. \\ To run the code, the following packages must be installed: scipy, tqdm, matplotlib.pyplot. The code takes the following arguments:
\begin{enumerate}
    \item \verb|undirected_graph|: boolean value indicating if the underlying graph is undirected,
    \item \verb|dataset_names|: the list of dataset names for which RCM is computed.
\end{enumerate}
and assumes that the datasets are in the .npz format and stored in \verb|./datasets/{dataset_name}_A.npz|. 

Upon execution, the code computes the RCM permutations, stores the permuted matrices in 

\verb|./datasets/{dataset_name}_A_CM_perm.npz|, \\ computes and prints the bandwidths and stores them in 

\verb|./datasets/bandwidth_{dataset_name}.txt|. \\
Next, it creates a plot of the RCM-permuted matrix and stores it in 

\verb|./datasets/CM_permutation_{dataset_name}.png|. \\ The code takes approximately ten to twenty minutes to run per dataset, depending on its structure.

\paragraph{A4. Dataset Analysis Code}
The graph statistics (\textbf{A4}) are computed in 

\verb|./scr/graphprocessing/graph_stats.py|. \\ This script requires the same packages and takes the argument \verb|dataset_names|  which has the same meaning as in \verb|rcm.py| (see description of \textbf{A3}). We assume that the datasets are in the .npz format and stored in 

\verb|./datasets/{dataset_name}_A.npz|. \\
Upon execution, the code prints graph statistics and stores them in 

\verb|./datasets/stats_{dataset_name}.txt|. \\ The code is expected to run within approximately ten  minutes per dataset.

The computed statistics should be identical with the data listed in Table 4.

%STOP_LATEX

\iffalse
\paragraph{A2. SpMM MPI Codes: Baseline 1.5D Algorithm}


The baseline 1.5D implementation is a variation of the state-of-the-art A-Stationary 1.5D SpMM algorithm~\cite{DBLP:conf/ics/SelvitopiBNTYB21}.
Assuming $P = P_iP_j$ available processes, we arrange them in a $P_i \times P_j$ Cartesian grid.
Each process has Cartesian coordinates $\left(i, j\right)$.
The sparse matrix $\mat{A}$ is similarly split into $P_iP_j$ 2D blocks, also with coordinates $\left(i, j\right)$, where $i \in 0..P_i - 1$, and $j \in 0..P_j - 1$.
The matrix $\mat{A}$ remains \textit{stationary}, meaning that each $\left(i, j\right)$ process holds the corresponding $\left(i, j\right)$ $\mat{A}$ block from start to finish. 
On the other hand, the dense matrices $\mat{X}$ and $\mat{Y}$ are split by rows into 1D blocks with some degree of replication, hence the term \textit{1.5D}.
It follows from the matrix multiplication algorithm that each $\left(i, j\right)$ process must receive the $j$-th $\mat{X}$ block,  multiply it with the $\left(i, j\right)$ $\mat{A}$ block, and contribute the partial sum to the $i$-th $\mat{Y}$ block.
Effectively, each $\mat{X}$ block must be replicated in the $P_i$ processes that share the same $j$-coordinate, while each $\mat{Y}$ block must be broken down to $P_j$ partial sums, originating from the $P_j$ processes that share the $i$-coordinate.

The difference between the algorithm described by Selvitopi et al. and our implementation lies in how and when the replication is realized.
The \mat{X} blocks are not initially replicated in the original algorithm, but each $\left(i, j\right)$ process starts with a unique sub-block.
To perform matrix multiplication, \textit{Allgather} collectives among the $P_i$ processes sharing the same $j$-coordinate are required to gather the entire $j$-th B block.
Similarly, at the end of the algorithm, \mat{Y} is not replicated.
Instead, each process holds the complete result for a unique sub-block.
This is achieved by \textit{Reduce\_scatter} collectives performed by the $P_j$ processes sharing the same $i$-coordinate.
We simplify the above scheme by assuming that the algorithm starts with \mat{X} already replicated and ends with \mat{Y} also fully replicated.
This allows the processes to start computing their partial sums immediately.
The replication of \mat{Y} is achieved with \textit{Allreduce} collectives among the processes that share the same $i$-coordinate.
Although the above algorithms are effectively the same when considering the data movement at a high level, they do not necessarily share latency and communication volume, depending on the exact $\alpha-\beta$ model used for the different collective operations.
\fi


\iffalse
\begin{table}[]
\caption{List of the datasets used in the paper with their downloading links.}
\vspace{-0.8em}
    \centering
    \def\arraystretch{1}
    \setlength\tabcolsep{0.7em}
    \begin{tabular}{|c|c|l|}
    \toprule
    Dataset & File Format  & URL  \\ \midrule
    MAWI  & .mat & \href{http://sparse.tamu.edu/MAWI}{Link}   \\
    GenBank & .mat & \href{https://sparse.tamu.edu/GenBank}{Link}  \\
    WebBase  & .mat& \href{http://sparse.tamu.edu/LAW/webbase-2001}{Link}  \\
    \bottomrule
    \end{tabular}
    \label{tab:dataset-links}
\end{table}
%STOP_LATEX

\fi
